Lattice Fermions Based on Higher-Dimensional Hyperdiamond Lattices

In this paper we generalize to higher dimensions several types of fermion actions on the hyperdiamond lattice including a two-parameter class of minimal-doubling fermions "Creutz fermion" and a simple fermion with sufficient discrete symmetry "BBTW fermion". Then it is shown that they possess some properties in common with the four-dimensional case: BBTW fermions in higher even dimensions inevitably yield unphysical degrees of freedom. Creutz fermions are defined on the distorted lattices, and they lose the high discrete symmetry of the original lattices. We also find properties specific to the higher-dimensional cases. The parameter range for Creutz action to yield minimal-doubling and physical fermions becomes narrower with the dimension getting higher, thus it becomes more and more difficult to realize minimal-doubling. In addition, we generalize the subspecies of Creutz and BBTW actions including a new class of minimal-doubling actions "Appended Creutz action".

==> honey_prim.tex <==
%WinTpicVersion3.08
\unitlength 0.1in
\begin{picture}( 17.3500, 13.4500)(  4.6500,-16.6000)
% LINE 2 0 3 0
% 2 1224 879 1411 987
% 
\special{pn 8}%
\special{pa 1224 880}%
\special{pa 1412 988}%
\special{fp}%
% LINE 2 0 3 0
% 2 1420 990 1420 1206
% 
\special{pn 8}%
\special{pa 1420 990}%
\special{pa 1420 1206}%
\special{fp}%
% LINE 2 0 3 0
% 2 1224 1311 1411 1203
% 
\special{pn 8}%
\special{pa 1224 1312}%
\special{pa 1412 1204}%
\special{fp}%
% LINE 2 0 3 0
% 2 1220 1311 1033 1203
% 
\special{pn 8}%
\special{pa 1220 1312}%
\special{pa 1034 1204}%
\special{fp}%
% LINE 2 0 3 0
% 2 1033 1203 1033 987
% 
\special{pn 8}%
\special{pa 1034 1204}%
\special{pa 1034 988}%
\special{fp}%
% LINE 2 0 3 0
% 2 1220 879 1033 987
% 
\special{pn 8}%
\special{pa 1220 880}%
\special{pa 1034 988}%
\special{fp}%
% LINE 2 0 3 0
% 2 1598 1311 1411 1203
% 
\special{pn 8}%
\special{pa 1598 1312}%
\special{pa 1412 1204}%
\special{fp}%
% LINE 2 0 3 0
% 2 1420 1206 1420 990
% 
\special{pn 8}%
\special{pa 1420 1206}%
\special{pa 1420 990}%
\special{fp}%
% LINE 2 0 3 0
% 2 1598 879 1411 987
% 
\special{pn 8}%
\special{pa 1598 880}%
\special{pa 1412 988}%
\special{fp}%
% LINE 2 0 3 0
% 2 1980 879 2167 987
% 
\special{pn 8}%
\special{pa 1980 880}%
\special{pa 2168 988}%
\special{fp}%
% LINE 2 0 3 0
% 2 2167 987 2167 1203
% 
\special{pn 8}%
\special{pa 2168 988}%
\special{pa 2168 1204}%
\special{fp}%
% LINE 2 0 3 0
% 2 1980 1311 2167 1203
% 
\special{pn 8}%
\special{pa 1980 1312}%
\special{pa 2168 1204}%
\special{fp}%
% LINE 2 0 3 0
% 2 1976 1311 1789 1203
% 
\special{pn 8}%
\special{pa 1976 1312}%
\special{pa 1790 1204}%
\special{fp}%
% LINE 2 0 3 0
% 2 1789 1203 1789 987
% 
\special{pn 8}%
\special{pa 1790 1204}%
\special{pa 1790 988}%
\special{fp}%
% LINE 2 0 3 0
% 2 1976 879 1789 987
% 
\special{pn 8}%
\special{pa 1976 880}%
\special{pa 1790 988}%
\special{fp}%
% LINE 2 0 3 0
% 2 846 879 1033 987
% 
\special{pn 8}%
\special{pa 846 880}%
\special{pa 1034 988}%
\special{fp}%
% LINE 2 0 3 0
% 2 1033 987 1033 1203
% 
\special{pn 8}%
\special{pa 1034 988}%
\special{pa 1034 1204}%
\special{fp}%
% LINE 2 0 3 0
% 2 846 1311 1033 1203
% 
\special{pn 8}%
\special{pa 846 1312}%
\special{pa 1034 1204}%
\special{fp}%
% LINE 2 0 3 0
% 2 842 1311 655 1203
% 
\special{pn 8}%
\special{pa 842 1312}%
\special{pa 656 1204}%
\special{fp}%
% LINE 2 0 3 0
% 2 655 1203 655 987
% 
\special{pn 8}%
\special{pa 656 1204}%
\special{pa 656 988}%
\special{fp}%
% LINE 2 0 3 0
% 2 842 879 655 987
% 
\special{pn 8}%
\special{pa 842 880}%
\special{pa 656 988}%
\special{fp}%
% LINE 2 0 3 0
% 2 1037 555 1224 663
% 
\special{pn 8}%
\special{pa 1038 556}%
\special{pa 1224 664}%
\special{fp}%
% LINE 2 0 3 0
% 2 1224 663 1224 879
% 
\special{pn 8}%
\special{pa 1224 664}%
\special{pa 1224 880}%
\special{fp}%
% LINE 2 0 3 0
% 2 1037 987 1224 879
% 
\special{pn 8}%
\special{pa 1038 988}%
\special{pa 1224 880}%
\special{fp}%
% LINE 2 0 3 0
% 2 1033 987 846 879
% 
\special{pn 8}%
\special{pa 1034 988}%
\special{pa 846 880}%
\special{fp}%
% LINE 2 0 3 0
% 2 846 879 846 663
% 
\special{pn 8}%
\special{pa 846 880}%
\special{pa 846 664}%
\special{fp}%
% LINE 2 0 3 0
% 2 1033 555 846 663
% 
\special{pn 8}%
\special{pa 1034 556}%
\special{pa 846 664}%
\special{fp}%
% LINE 2 0 3 0
% 2 1793 555 1980 663
% 
\special{pn 8}%
\special{pa 1794 556}%
\special{pa 1980 664}%
\special{fp}%
% LINE 2 0 3 0
% 2 1980 663 1980 879
% 
\special{pn 8}%
\special{pa 1980 664}%
\special{pa 1980 880}%
\special{fp}%
% LINE 2 0 3 0
% 2 1793 987 1980 879
% 
\special{pn 8}%
\special{pa 1794 988}%
\special{pa 1980 880}%
\special{fp}%
% LINE 2 0 3 0
% 2 1789 987 1602 879
% 
\special{pn 8}%
\special{pa 1790 988}%
\special{pa 1602 880}%
\special{fp}%
% LINE 2 0 3 0
% 2 1602 879 1602 663
% 
\special{pn 8}%
\special{pa 1602 880}%
\special{pa 1602 664}%
\special{fp}%
% LINE 2 0 3 0
% 2 1789 555 1602 663
% 
\special{pn 8}%
\special{pa 1790 556}%
\special{pa 1602 664}%
\special{fp}%
% LINE 2 0 3 0
% 2 1415 555 1602 663
% 
\special{pn 8}%
\special{pa 1416 556}%
\special{pa 1602 664}%
\special{fp}%
% LINE 2 0 3 0
% 2 1602 663 1602 879
% 
\special{pn 8}%
\special{pa 1602 664}%
\special{pa 1602 880}%
\special{fp}%
% LINE 2 0 3 0
% 2 1415 987 1602 879
% 
\special{pn 8}%
\special{pa 1416 988}%
\special{pa 1602 880}%
\special{fp}%
% LINE 2 0 3 0
% 2 1411 987 1224 879
% 
\special{pn 8}%
\special{pa 1412 988}%
\special{pa 1224 880}%
\special{fp}%
% LINE 2 0 3 0
% 2 1224 879 1224 663
% 
\special{pn 8}%
\special{pa 1224 880}%
\special{pa 1224 664}%
\special{fp}%
% LINE 2 0 3 0
% 2 1411 555 1224 663
% 
\special{pn 8}%
\special{pa 1412 556}%
\special{pa 1224 664}%
\special{fp}%
% LINE 2 0 3 0
% 2 1037 1203 1224 1311
% 
\special{pn 8}%
\special{pa 1038 1204}%
\special{pa 1224 1312}%
\special{fp}%
% LINE 2 0 3 0
% 2 1224 1311 1224 1527
% 
\special{pn 8}%
\special{pa 1224 1312}%
\special{pa 1224 1528}%
\special{fp}%
% LINE 2 0 3 0
% 2 1037 1635 1224 1527
% 
\special{pn 8}%
\special{pa 1038 1636}%
\special{pa 1224 1528}%
\special{fp}%
% LINE 2 0 3 0
% 2 1033 1635 846 1527
% 
\special{pn 8}%
\special{pa 1034 1636}%
\special{pa 846 1528}%
\special{fp}%
% LINE 2 0 3 0
% 2 846 1527 846 1311
% 
\special{pn 8}%
\special{pa 846 1528}%
\special{pa 846 1312}%
\special{fp}%
% LINE 2 0 3 0
% 2 1033 1203 846 1311
% 
\special{pn 8}%
\special{pa 1034 1204}%
\special{pa 846 1312}%
\special{fp}%
% LINE 2 0 3 0
% 2 1415 1203 1602 1311
% 
\special{pn 8}%
\special{pa 1416 1204}%
\special{pa 1602 1312}%
\special{fp}%
% LINE 2 0 3 0
% 2 1602 1311 1602 1527
% 
\special{pn 8}%
\special{pa 1602 1312}%
\special{pa 1602 1528}%
\special{fp}%
% LINE 2 0 3 0
% 2 1415 1635 1602 1527
% 
\special{pn 8}%
\special{pa 1416 1636}%
\special{pa 1602 1528}%
\special{fp}%
% LINE 2 0 3 0
% 2 1411 1635 1224 1527
% 
\special{pn 8}%
\special{pa 1412 1636}%
\special{pa 1224 1528}%
\special{fp}%
% LINE 2 0 3 0
% 2 1224 1527 1224 1311
% 
\special{pn 8}%
\special{pa 1224 1528}%
\special{pa 1224 1312}%
\special{fp}%
% LINE 2 0 3 0
% 2 1411 1203 1224 1311
% 
\special{pn 8}%
\special{pa 1412 1204}%
\special{pa 1224 1312}%
\special{fp}%
% LINE 2 0 3 0
% 2 1793 1203 1980 1311
% 
\special{pn 8}%
\special{pa 1794 1204}%
\special{pa 1980 1312}%
\special{fp}%
% LINE 2 0 3 0
% 2 1980 1311 1980 1527
% 
\special{pn 8}%
\special{pa 1980 1312}%
\special{pa 1980 1528}%
\special{fp}%
% LINE 2 0 3 0
% 2 1793 1635 1980 1527
% 
\special{pn 8}%
\special{pa 1794 1636}%
\special{pa 1980 1528}%
\special{fp}%
% LINE 2 0 3 0
% 2 1789 1635 1602 1527
% 
\special{pn 8}%
\special{pa 1790 1636}%
\special{pa 1602 1528}%
\special{fp}%
% LINE 2 0 3 0
% 2 1602 1527 1602 1311
% 
\special{pn 8}%
\special{pa 1602 1528}%
\special{pa 1602 1312}%
\special{fp}%
% LINE 2 0 3 0
% 2 1789 1203 1602 1311
% 
\special{pn 8}%
\special{pa 1790 1204}%
\special{pa 1602 1312}%
\special{fp}%
% CIRCLE 2 0 0 0
% 4 655 987 655 962 655 962 655 962
% 
\special{pn 8}%
\special{sh 0.600}%
\special{ar 656 988 26 26  0.0000000 6.2831853}%
% CIRCLE 2 0 0 0
% 4 1033 987 1033 962 1033 962 1033 962
% 
\special{pn 8}%
\special{sh 0.600}%
\special{ar 1034 988 26 26  0.0000000 6.2831853}%
% CIRCLE 2 0 0 0
% 4 1411 987 1411 962 1411 962 1411 962
% 
\special{pn 8}%
\special{sh 0.600}%
\special{ar 1412 988 26 26  0.0000000 6.2831853}%
% CIRCLE 2 0 0 0
% 4 1789 987 1789 962 1789 962 1789 962
% 
\special{pn 8}%
\special{sh 0.600}%
\special{ar 1790 988 26 26  0.0000000 6.2831853}%
% CIRCLE 2 0 0 0
% 4 2167 987 2167 962 2167 962 2167 962
% 
\special{pn 8}%
\special{sh 0.600}%
\special{ar 2168 988 26 26  0.0000000 6.2831853}%
% CIRCLE 2 0 0 0
% 4 1789 1635 1789 1610 1789 1610 1789 1610
% 
\special{pn 8}%
\special{sh 0.600}%
\special{ar 1790 1636 26 26  0.0000000 6.2831853}%
% CIRCLE 2 0 0 0
% 4 1411 1635 1411 1610 1411 1610 1411 1610
% 
\special{pn 8}%
\special{sh 0.600}%
\special{ar 1412 1636 26 26  0.0000000 6.2831853}%
% CIRCLE 2 0 0 0
% 4 1033 1635 1033 1610 1033 1610 1033 1610
% 
\special{pn 8}%
\special{sh 0.600}%
\special{ar 1034 1636 26 26  0.0000000 6.2831853}%
% CIRCLE 2 0 2 0
% 4 1033 555 1033 530 1033 530 1033 530
% 
\special{pn 8}%
\special{sh 0}%
\special{ar 1034 556 26 26  0.0000000 6.2831853}%
% CIRCLE 2 0 2 0
% 4 1411 555 1411 530 1411 530 1411 530
% 
\special{pn 8}%
\special{sh 0}%
\special{ar 1412 556 26 26  0.0000000 6.2831853}%
% CIRCLE 2 0 2 0
% 4 1789 555 1789 530 1789 530 1789 530
% 
\special{pn 8}%
\special{sh 0}%
\special{ar 1790 556 26 26  0.0000000 6.2831853}%
% CIRCLE 2 0 2 0
% 4 1980 1527 1980 1502 1980 1502 1980 1502
% 
\special{pn 8}%
\special{sh 0}%
\special{ar 1980 1528 26 26  0.0000000 6.2831853}%
% CIRCLE 2 0 2 0
% 4 1602 1527 1602 1502 1602 1502 1602 1502
% 
\special{pn 8}%
\special{sh 0}%
\special{ar 1602 1528 26 26  0.0000000 6.2831853}%
% CIRCLE 2 0 2 0
% 4 1224 1527 1224 1502 1224 1502 1224 1502
% 
\special{pn 8}%
\special{sh 0}%
\special{ar 1224 1528 26 26  0.0000000 6.2831853}%
% CIRCLE 2 0 2 0
% 4 846 1527 846 1502 846 1502 846 1502
% 
\special{pn 8}%
\special{sh 0}%
\special{ar 846 1528 26 26  0.0000000 6.2831853}%
% CIRCLE 2 0 2 0
% 4 846 879 846 854 846 854 846 854
% 
\special{pn 8}%
\special{sh 0}%
\special{ar 846 880 26 26  0.0000000 6.2831853}%
% CIRCLE 2 0 2 0
% 4 1224 879 1224 854 1224 854 1224 854
% 
\special{pn 8}%
\special{sh 0}%
\special{ar 1224 880 26 26  0.0000000 6.2831853}%
% CIRCLE 2 0 2 0
% 4 1602 879 1602 854 1602 854 1602 854
% 
\special{pn 8}%
\special{sh 0}%
\special{ar 1602 880 26 26  0.0000000 6.2831853}%
% CIRCLE 2 0 2 0
% 4 1980 879 1980 854 1980 854 1980 854
% 
\special{pn 8}%
\special{sh 0}%
\special{ar 1980 880 26 26  0.0000000 6.2831853}%
% CIRCLE 2 0 0 0
% 4 846 660 846 634 846 634 846 634
% 
\special{pn 8}%
\special{sh 0.600}%
\special{ar 846 660 26 26  0.0000000 6.2831853}%
% CIRCLE 2 0 2 0
% 4 2170 1200 2170 1170 2170 1170 2170 1170
% 
\special{pn 8}%
\special{sh 0}%
\special{ar 2170 1200 30 30  0.0000000 6.2831853}%
% CIRCLE 2 0 2 0
% 4 1790 1200 1790 1170 1790 1170 1790 1170
% 
\special{pn 8}%
\special{sh 0}%
\special{ar 1790 1200 30 30  0.0000000 6.2831853}%
% CIRCLE 2 0 2 0
% 4 1410 1200 1410 1170 1410 1170 1410 1170
% 
\special{pn 8}%
\special{sh 0}%
\special{ar 1410 1200 30 30  0.0000000 6.2831853}%
% CIRCLE 2 0 2 0
% 4 1030 1200 1030 1170 1030 1170 1030 1170
% 
\special{pn 8}%
\special{sh 0}%
\special{ar 1030 1200 30 30  0.0000000 6.2831853}%
% CIRCLE 2 0 2 0
% 4 660 1200 660 1170 660 1170 660 1170
% 
\special{pn 8}%
\special{sh 0}%
\special{ar 660 1200 30 30  0.0000000 6.2831853}%
% CIRCLE 2 0 0 0
% 4 1980 660 1980 630 1980 630 1980 630
% 
\special{pn 8}%
\special{sh 0.600}%
\special{ar 1980 660 30 30  0.0000000 6.2831853}%
% CIRCLE 2 0 0 0
% 4 1600 660 1600 630 1600 630 1600 630
% 
\special{pn 8}%
\special{sh 0.600}%
\special{ar 1600 660 30 30  0.0000000 6.2831853}%
% CIRCLE 2 0 0 0
% 4 1220 660 1220 630 1220 630 1220 630
% 
\special{pn 8}%
\special{sh 0.600}%
\special{ar 1220 660 30 30  0.0000000 6.2831853}%
% STR 2 0 3 0
% 3 1620 1030 1620 1080 5 0
% a$^2$
\put(16.2000,-10.8000){\makebox(0,0){a$^2$}}%
% VECTOR 0 0 3 0
% 2 1435 1175 1585 910
% 
\special{pn 20}%
\special{pa 1436 1176}%
\special{pa 1586 910}%
\special{fp}%
\special{sh 1}%
\special{pa 1586 910}%
\special{pa 1536 958}%
\special{pa 1560 956}%
\special{pa 1570 978}%
\special{pa 1586 910}%
\special{fp}%
% VECTOR 0 0 3 0
% 2 1385 1175 1235 915
% 
\special{pn 20}%
\special{pa 1386 1176}%
\special{pa 1236 916}%
\special{fp}%
\special{sh 1}%
\special{pa 1236 916}%
\special{pa 1252 984}%
\special{pa 1262 962}%
\special{pa 1286 964}%
\special{pa 1236 916}%
\special{fp}%
% STR 2 0 3 0
% 3 1220 1030 1220 1080 5 0
% a$^1$
\put(12.2000,-10.8000){\makebox(0,0){a$^1$}}%
% STR 2 0 3 0
% 3 600 300 600 400 5 0
% (c)
\put(6.0000,-4.0000){\makebox(0,0){(c)}}%
% CIRCLE 2 0 0 0
% 4 1980 1310 1980 1280 1980 1280 1980 1280
% 
\special{pn 8}%
\special{sh 0.600}%
\special{ar 1980 1310 30 30  0.0000000 6.2831853}%
% CIRCLE 2 0 0 0
% 4 1600 1310 1600 1280 1600 1280 1600 1280
% 
\special{pn 8}%
\special{sh 0.600}%
\special{ar 1600 1310 30 30  0.0000000 6.2831853}%
% CIRCLE 2 0 0 0
% 4 1220 1310 1220 1280 1220 1280 1220 1280
% 
\special{pn 8}%
\special{sh 0.600}%
\special{ar 1220 1310 30 30  0.0000000 6.2831853}%
% CIRCLE 2 0 0 0
% 4 850 1310 850 1280 850 1280 850 1280
% 
\special{pn 8}%
\special{sh 0.600}%
\special{ar 850 1310 30 30  0.0000000 6.2831853}%
\end{picture}%

